iCrawl: Improving the Freshness of Web Collections by Integrating Social Web and Focused Web Crawling

Researchers in the Digital Humanities and journalists need to monitor, collect and analyze fresh online content regarding current events such as the Ebola outbreak or the Ukraine crisis on demand. However, existing focused crawling approaches only consider topical aspects while ignoring temporal aspects and therefore cannot achieve thematically coherent and fresh Web collections. Especially Social Media provide a rich source of fresh content, which is not used by state-of-the-art focused crawlers. In this paper we address the issues of enabling the collection of fresh and relevant Web and Social Web content for a topic of interest through seamless integration of Web and Social Media in a novel integrated focused crawler. The crawler collects Web and Social Media content in a single system and exploits the stream of fresh Social Media content for guiding the crawler.

==> input/analysis-components.tex <==
% \section{Crawl Focusing Strategies}
% \label{sec:crawl_focussing_strategies}

The extended capabilities of the iCrawl system require that we perform a semantic analysis of the crawled data, 
especially for focusing the crawl and for providing the crawl monitoring interface.
This is in contrast to standard Web crawlers which only need to analyze the data to extract links to new pages.
The iCrawl semantic analysis occurs in the \emph{Online Analysis Module} that 
performs a shallow analysis during the crawl for use by the focusing and 
monitoring components.
   
The purpose of the online analysis module is twofold: On the one hand it provides relevance scores for 
crawled documents and their outgoing links based on their similarity to the crawl specification, which 
allow the crawler to decide if and in which order uncrawled URLs should be downloaded.
On the other hand it also provides prompt feedback to the user about the content of the crawled documents.

The online analysis is conducted on each crawled document and therefore needs to be able to process documents 
at approximately the rate they are downloaded. This allows only a shallow analysis of the crawled data.
In particular, any I/O operation, \eg to query external data sources, are forbidden 
and also only one document at a time can be considered.

For each fetched page the module extracts and stores named entities and relevant keywords that occur 
on that page, together with a link back to this source page and snippets that show the context of the entity.
This information is particularly helpful for the monitoring task: By looking at the frequency of entities 
in the crawl over time, the user can get an idea about the development of the crawl.
The Monitoring UI can also provide additional context for the most frequent entities by showing co-occurring 
keywords and text snippets, which aids the understanding of those entities.

For the prioritization we compute a relevance score based on the similarity between the extracted information 
and the crawl specification. This can be done by measuring the textual overlap between keywords specified by 
the user and the entity labels. However, the keywords by the user may not match the actual content of the 
pages, \eg when synonyms are used. This would lead the crawler to ignore such content, even if it is highly 
relevant. To address this issue, we extend the crawl specification using topic expansion techniques which 
have been studied extensively in Information Retrieval (\eg for query 
expansion \cite{survey:queryExpansion:2012}). The overlap calculation between content extracted from Web 
pages and the crawl specification is then done on the expanded content.

As described above, the online analysis module has to satisfy strict speed requirements.
This prohibits the use of most Named Entity Recognition (NER) systems, especially those that link entity 
to external knowledge bases. Fortunately, some recent NER systems such as SpeedRead~\cite{speedread} focus 
on fast processing times (up to ten times faster than other state-of-the-art systems), while maintaining a 
good accuracy. The labels of entities extracted in this way are used in the monitoring UI together with 
simple statistics about the frequency of the entity and the number of documents it occurs in.
In this way the online analysis and monitoring components can be implemented with a high performance.



==> input/focusing.tex <==
\section{Focusing and Prioritization of Integrated Crawls}
\label{sec:focusing}

% Focused crawling starts with the manual definition of the \textit{crawl specification}:
% a list of seed URLs, keywords and (optionally) entities representing
% the topical focus of the crawl. The crawl specification is necessary for the focused
% crawler to efficiently find relevant pages and to judge their relevance automatically. 
% %
% To this extent, we represent the crawl specification as a vector, called \textit{reference vector}, 
% primarily containing terms extracted from the seed documents as well as user-defined keywords and entities. 
% We describe the term weighting scheme in Section \ref{sec:document-vector}.

In order to efficiently perform the crawling process, we need to ensure that only the 
URLs expected to be relevant to the topical focus of the crawl
%crawl specification 
are downloaded and the URLs that are likely to be irrelevant are discarded.
This is done through the \emph{prioritization process} that orders the URLs in the crawler 
queue by their decreasing relevance score.
%
%TODO: refer to relevance score in the formulas
%

In order to enable efficient automatic relevance estimation,
we represent the crawl specification as a term vector, called the \textit{reference vector}.
Then, we use the cosine similarity to the reference vector as a relevance estimate. 
%
We describe the term weighting scheme for the reference and document vectors in Section \ref{sec:document-vector}
and the relevance score estimation for the URLs in Section \ref{sec:outlink-relevance-es}.

%
%Then, we can use similarity measures to relevance with respect to the 


%
% TODO: that should not be called document. We create CS vector and then link context vectors.
% It also does not say how the seed vectors are aggregated to one CS vector.
% Btw, it should be sufficient to boost the terms only in the CS vector.
%
\subsection{Crawl Specification and Document Vectors}
\label{sec:document-vector}

The crawl specification in iCrawl contains
a list of seeds (URLs and Social Media queries) and keywords that best 
describe the topical focus of the crawl from the user's point of view. 
%
To enable efficient processing, the crawl specification is represented as a reference vector.
To construct this vector we tokenize and stem the text of the documents referred by the seed URLs 
and remove the stop words using language-specific analyzers from the Lucene Java 
library.\footnote{\url{http://lucene.apache.org/core/}}
The terms obtained this way are weighted by their frequencies in the seed documents.
%
% How are they aggregated? Just a sum or any normalization?
% 
As previous work has shown bigrams to be effective for crawl focusing \citep{Laranjeira2014}, 
also use in the vector term bigrams in addition to the terms.
%
As we do not have a reference collection of comparable documents during the crawl, we do not use any features
based on document frequency. 

The weights of the terms representing keywords explicitly defined in the crawl 
specification are boosted. 
This helps the crawler disambiguate seed pages containing multiple topics by shifting the reference vector towards the expected interpretation.
To perform boosting, we check the overlap of each term with the keywords, 
as terms (in the case of bigrams) can contain multiple tokens. 
Based on whether there is a partial or full overlap, 
we assign a \emph{term weight} $tw_t$ to the term $t$ in the document vector as follows:
\begin{equation}
  \label{eq:term-weight}
  tw_t = 
    \begin{cases}
      w_f & \text{if $t$ is fully contained in a keyword,} \\
      w_p & \text{if $t$ is partially contained in a keyword,} \\
      w_d & \text{otherwise.}
    \end{cases}
\end{equation}
Finally, the term weight obtained this way is multiplied with the term frequency. 
In our evaluation, we experimentally set the values 
for $w_f$, $w_p$ and $w_d$ to $2$, $1.5$ and $1$, respectively.

The document vectors used to perform the relevance estimation for URLs 
are constructed analogously to the reference vector. 


%\subsection{Outlink Relevance Score Estimation}
\subsection{Relevance Estimation for URLs}
\label{sec:outlink-relevance-es}

In general, the relevance of a URL to the topical focus of the crawl
(represented by the crawl specification)
can be estimated using the content of the document referenced by the URL, 
the structure of the link graph, the crawling history, as well as the URL context in the linking pages. 
As the content of the document referenced by the URL is not available before fetching, iCrawl has to estimate 
the relevance based on the features external to the document.
%
Generally, systems that possess crawling history can use link graph structure
(e.g. PageRank \cite{pageRank}) or the content of the previously downloaded versions of the URLs to perform relevance 
estimation. However, these history-based features are not available for our use cases. 
%
Therefore, we use only the pages that are known to the crawler from the current crawling process 
and estimate the relevance of their outlinks based on the link context. 
%

Although a relevant Web document can contain many outlinks, not all of them are always relevant for the crawl.
Examples of irrelevant links include the site navigation links and advertisements.
We therefore need to compute the relevance score for each individual outlink.
This can be achieved by using the context of the links in the document.
The features based on the link context rely on the assumption that pages link to other 
pages that are topically related and provide a descriptive anchor text, 
whereas anchor text is understood in a broad sense here.

The textual context of the links can differ in granularity.
In particular, we can use the anchor text or the surrounding text of the link \cite{pant_deriving_2003}.
Either of those may still contain only irrelevant text such as ``click here''.
We therefore combine both features and add the relevance of the entire document as a last resort.

Each feature is implemented by creating a document vector from the selected parts of the document 
and calculating the cosine similarity to the reference vector. This method is very computationally 
efficient and has proven to be effective in many areas of Information Retrieval~{\cite{manning2008}}.

For the \emph{anchor similarity} $w_a(l_i)$ of each link $l_i$ we extract the text of all HTML \texttt{<A \ldots{>}} tags 
referencing $l_i$.
For the \emph{paragraph similarity} $w_p(l_i)$ we extract the content of the paragraph surrounding each relevant link.
A paragraph is here defined as an HTML block element that contains at least $\rho$ word tokens.
The \emph{document similarity} $w_d$ is computed using the text of the entire document.
We combine the three similarity scores using a linear combination to derive the relevance score $w(l_i)$ for each outlink:
\begin{equation}
  \label{eq:link-relevance}
  w(l_i) = \lambda_a w_a(l_i) + \lambda_p w_p(l_i) + \lambda_d w_d,
\end{equation}
where $ \lambda_a + \lambda_p + \lambda_d = 1$.
In our experiment, we experimentally set $\lambda_a = \lambda_p = \lambda_d = \frac13$ and chose a minimum paragraph size $\rho$ of $50$.

Finally, a URL can be linked to from many different pages.
The final relevance score of a URL is therefore computed as the sum of the relevance scores provided 
by each individual inlinking page.
This ensures that popular URLs are crawled with a higher priority.
After a page is processed, the relevance score of each unfetched outlink is  
updated and its position in the queue is adjusted accordingly.

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../icrawl_www15"
%%% End: 


==> input/freshness.tex <==
\section{Estimating Freshness of\\Web Content}
\label{sec:freshness}

%define freshness, separate from web search definition

Along with the topical relevance, the freshness of the collected pages is one of the crucial requirements of 
journalists and researchers, who are interested in irregular crawls on current events and topics performed 
on demand. In this context, it is important to automatically guide the crawler towards relevant and fresh content and to estimate freshness of the crawled pages efficiently and accurately.
%

If a page has been previously crawled, its freshness can be estimated using the crawl history. This history is typically obtained by regular unfocused large-scale crawls and can provide the date the document has been discovered by the crawler (inception date).
This approach is used in many of the larger organizations in the field of Web crawling such as Web search engines and Web archiving institutions.

% The iCrawl is a personal tool for journalists and researchers, who are interested in 
% irregular crawls on current events and topics on demand. 
As the iCrawl users (journalists and researchers) typically do not have the infrastructure required for regular large-scale Web crawls, freshness measures relying on the crawl history are not applicable.
%
In order to directly provide Web crawler with the entry points to the fresh Web content, we exploit the idea of an integrated Web and Social Media crawling. To assess page freshness, we rely on the content-based creation date estimates and compute the difference between the fetch time and the (estimated) page creation time.

\begin{mydef}
\label{def:freshness}
\textbf{Page Freshness:} If page $P$ was fetched at time $t_{f}$ and the (estimated) time of the creation 
of this page is $t_{c}$, then the freshness $F_{P}$ of $P$ is proportional to the length of the time interval between the fetch time and the estimated creation time: $F_{P} \approx t_{f} - t_{c}$.
\end{mydef} 


Content-based estimation of Web page creation time faces technical challenges as such information is highly 
syntactically heterogeneous (and is not always explicitly available). Moreover, Web pages do not offer reliable 
metadata concerning their creation date \cite{Tannier14}. 
In order to allow an efficient freshness evaluation, 
we rely on several content-based features (presented in Section~\ref{sec:evaluation}
in more detail).
%regular expressions. 
Other possibilities for estimation of creation date include usage of existing tools such as 
DCTFinder \cite{Tannier14} that combine rule-based approaches with probabilistic models. 
% and achieve high precision.



%TODO: @Gerhard: more details in the evaluation section 
% How is it done for social media freshness?





%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../icrawl_www15"
%%% End: 


==> input/tab-domains-ukraine.tex <==

  \begin{tabular}{lrrrlrrr}
\toprule
\multicolumn{4}{c}{Twitter-based} & 
\multicolumn{4}{c}{Unfocused} \\
\cmidrule(lr){1-4}
\cmidrule(lr){5-8}

Domain & Avg rel. & Avg freshness & Freq &
Domain & Avg rel. & Avg freshness & Freq \\

         youtube.com	& 0.11	&  3,988.86	& 1712 	&          reuters.com	& 0.12	&  5,891.42	& 1827 \\
       instagram.com	& 0.01	&         ?	& 891 	&          twitter.com	& 0.04	&  1,000.32	& 1113 \\
        facebook.com	& 0.07	&    449.32	& 805 	&             time.com	& 0.20	&  1,831.79	& 781 \\ 
        kyivpost.com	& 0.56	&  5,523.39	& 519 	&               rt.com	& 0.13	&  7,078.81	& 729 \\ 
     edsonide.med.br	& 0.01	&    202.88	& 459 	&           google.com	& 0.06	&  2,018.34	& 613 \\ 
          linkis.com	& 0.12	&     64.90	& 457 	&         kyivpost.com	& 0.50	&  8,849.28	& 532 \\ 
           jabry.com	& 0.01	&  1,499.16	& 441 	&      theguardian.com	& 0.21	&  2,728.06	& 510 \\ 
         twitter.com	& 0.05	&     77.03	& 437 	&   thomsonreuters.com	& 0.08	& 10,385.13	& 215 \\ 
           yahoo.com	& 0.32	&     45.83	& 394 	&        microsoft.com	& 0.09	&  2,713.00	& 168 \\ 
       wordpress.com	& 0.23	&    549.21	& 378 	&          youtube.com	& 0.02	& 40,704.67	& 153 \\ 

\bottomrule                                              

\addlinespace


\toprule
\multicolumn{4}{c}{Focused} & 
\multicolumn{4}{c}{Integrated} \\
\cmidrule(lr){1-4}
\cmidrule(lr){5-8}
Domain & Avg rel. & Avg freshness & Freq &
Domain & Avg rel. & Avg freshness & Freq \\
\cmidrule(lr){1-4}
\cmidrule(lr){5-8}

       wikipedia.org	& 0.11	& 18,822.77	& 9959	&       wikipedia.org	& 0.11	& 18,671.14	& 12519 \\
     theguardian.com	& 0.18	&  9,510.90	& 8974	&     theguardian.com	& 0.18	& 10,099.87	& 10566 \\
            time.com	& 0.19	&  4,266.94	& 3604	&            time.com	& 0.19	&  4,404.56	& 3973 	\\
         mozilla.org	& 0.09	& 13,467.77	& 2808	&         twitter.com	& 0.04	&  4,655.66	& 2667 	\\
         twitter.com	& 0.04	&  2,795.87	& 2343	&         reuters.com	& 0.17	& 10,639.19	& 2009 	\\
         reuters.com	& 0.18	&  9,479.94	& 2116	&       jmcolberg.com	& 0.04	& 55,239.86	& 1977 	\\
              rt.com	& 0.20	&  7,945.52	& 1792	&              rt.com	& 0.21	&  7,034.99	& 1693 	\\
       jmcolberg.com	& 0.04	& 57,043.67	& 1702	&       usembassy.gov	& 0.06	& 12,894.11	& 1685  \\
       usembassy.gov	& 0.07	& 14,159.00	& 1561	&        kyivpost.com	& 0.53	&  7,233.13	& 1439  \\
        kyivpost.com	& 0.53	&  6,650.35	& 1102	&            cnet.com	& 0.08	& 12,262.19	& 1143  \\

\bottomrule
\end{tabular}


==> input/tab-domains-ukraine2.tex <==

  \begin{tabular}{lrrrlrrr}
\toprule
\multicolumn{4}{c}{Twitter-based} & 
\multicolumn{4}{c}{Unfocused} \\
\cmidrule(lr){1-4}
\cmidrule(lr){5-8}

Domain & Avg rel. & Avg freshness & Freq &
Domain & Avg rel. & Avg freshness & Freq \\
\cmidrule(lr){1-4}
\cmidrule(lr){5-8}

         youtube.com	& 0.11	&  4,411.26	& 1022	&          reuters.com	& 0.18	&  9,040.30	& 1398 \\
    hosting-test.net	& 0.01	&  4,750.71	& 792	&               rt.com	& 0.23	& 10,502.07	& 1042 \\
            nvua.net	& 0.02	&    281.82	& 533	&         kyivpost.com	& 0.50	&  7,088.94	& 981 \\ 
       instagram.com	& 0.00	&         ?	& 374	&            pehub.com	& 0.12	&  5,253.42	& 412 \\ 
        facebook.com	& 0.06	&  2,038.76	& 323	&      theguardian.com	& 0.23	&  8,617.10	& 406 \\ 
          linkis.com	& 0.12	&    114.13	& 237	&          nytimes.com	& 0.17	&  7,466.89	& 369 \\ 
       priobreti.com	& 0.02	&    192.52	& 237	&           google.com	& 0.05	&  2,166.70	& 223 \\ 
         blogspot.de	& 0.18	&  3,696.68	& 212	&        microsoft.com	& 0.11	&  7,304.67	& 221 \\ 
         twitter.com	& 0.05	&    182.15	& 187	&            apple.com	& 0.09	&  4,617.12	& 181 \\ 
               co.vu	& 0.04	&         ?	& 184	&             time.com	& 0.25	&  1,425.97	& 167 \\ 
                                                                                                                   

\bottomrule                                              

\addlinespace


\toprule
\multicolumn{4}{c}{Focused} & 
\multicolumn{4}{c}{Integrated} \\
\cmidrule(lr){1-4}
\cmidrule(lr){5-8}
Domain & Avg rel. & Avg freshness & Freq &
Domain & Avg rel. & Avg freshness & Freq \\
\cmidrule(lr){1-4}
\cmidrule(lr){5-8}

              rt.com	& 0.26	&  2,462.81	& 163	&               rt.com	& 0.29	& 12,948.36	& 231 \\
       wikipedia.org	& 0.23	& 30,490.60	& 156	&               ria.ru	& 0.34	&  1,479.70	& 206 \\
       wordpress.com	& 0.25	&    174.80	& 121	&        wordpress.com	& 0.26	&    260.95	& 205 \\
              ria.ru	& 0.32	&  1,472.59	& 118	&         kyivpost.com	& 0.51	&  7,189.10	& 196 \\
     theguardian.com	& 0.30	&  1,146.99	& 113	&      theguardian.com	& 0.31	&    991.44	& 189 \\
        kyivpost.com	& 0.50	&  5,144.32	& 110	&        wikipedia.org	& 0.26	& 31,090.30	& 127 \\
           yahoo.com	& 0.20	&    486.17	&  95	&            yahoo.com	& 0.22	&    562.05	& 121 \\
           rferl.org	& 0.25	&     84.66	&  75	&        instagram.com	& 0.00	&         ?	& 103 \\
         nytimes.com	& 0.16	&    976.05	&  65	&  euromaidanpress.com	& 0.39	&    198.15	&  95 \\
         reuters.com	& 0.26	&    601.96	&  64	&             time.com	& 0.30	&  1,142.55	&  95 \\

\bottomrule
\end{tabular}


==> input/usecases.tex <==

\section{Motivation and Requirements}
\label{sec:use-cases-requ}


Our user requirements study in \cite{icrawlRequirements} revealed that more and more disciplines are interested in 
mining and analyzing the Web. User-generated content and especially the Social Web is attractive for many humanities 
disciplines. Also journalists are interested in the content as it provides a direct access to the people's views 
about politics, popular topics, events or entities shared on Social Media platforms. 

The increasing availability of tools and methods for processing masses of data within short time, 
e.g. Apache Hadoop, enables an efficient analysis of content. However, such an analysis of content requires 
to have the content stored in easy accessible collections and not distributed across the Web. Therefore Web 
crawlers for Web collection creation are gaining more interest. For a long time this was a niche activity mainly 
conducted by Internet Archives or National Libraries. As a consequence Web crawlers were optimized for their 
needs namely harvesting of whole domains. This increasing interest to analyze and understand events or entities 
the creation of focused Web collections on a case by case basis gained more importance and changes the requirements 
for Web crawlers. Instead of crawling whole domains current Web collection crawlers need to be guided by topics and events. 


\subsubsection*{Use Case: Social Sciences}

The aim of the social sciences is to understand the society and the relationships among individuals within the society. The importance of digital data analysis for social research has been recognized especially in the sub-field of digital sociology~\cite{DL2012}. 

Starting points could be regular shallow observation crawls of major news sites for identifying interesting topics for research. Once the topic has been identified, focused crawls around the topic in official, journalistic sources as well as Social Media should be conducted. Especially with respect to controversial topics, such as immigration, education and social inequality, the collected resources can represent the diversity of opinions on the topic in various online sources thus facilitating sociological research in this area. In contrast, the lack of representation of a topic in online media sources can indicate general lack of interest towards this topic.

\subsubsection*{Derived Requirements}

Beside the topical aspects the authenticity and context of content are other important requirements by the users. Crawled information should not only be as authentic as possible from the layout and presentation but also from the embedded information like embedded Twitter feeds. Vice versa collected tweets from Twitter with embedded links need should also present the linked page to understand the context of the tweet. But the Web and Social Web is ephemeral and under constant evolution. Pages can quickly change are become unreachable even within hours.

Today's approaches with loosely coupled crawlers can easily lead to big time gaps between the publication of page or message, the collection of the content and linked or embedded content. The shorter the time gap the fresher the content in the collection. Consequently to build most authentic and comprehensive Web collection the freshness should be as high as possible. By limiting the time gaps the authenticity of content can greatly be improved.




%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "..//icrawl_www15"
%%% End: 

